A model predictive control (MPC)-integrated multiphase immersed boundary (IB) framework for simulating wave energy converters (WECs)

In this work, we present a novel MPC-integrated multiphase IB framework that can compute the optimal energy-maximizing control force on-the-fly by dynamically interacting with a high-fidelity numerical wave tank (NWT). Due to the requirement of solving a constrained optimization problem at each time step of the IB simulation, the MPC algorithm utilizes a low-dimensional dynamical model of the device that is based on the linear potential theory (LPT). The multiphase IB solver, on the other hand, is based on the high-dimensional fictitious domain Brinkman penalization (FD/BP) method, which fully-resolves the hydrodynamic nonlinearities associated with the wave-structure interaction (WSI). A time-series forecasting auto-regressive model is implemented that predicts wave heights to estimate the future wave excitation/Froude- Krylov forces for the MPC algorithm. Moreover, we also experiment with non-linear Froude-Krylov (NLFK) forces for the first time in an MPC formulation. Under varying sea conditions, the predictions of the MPC-integrated multiphase IB solver are compared to the widely popular LPT-based solvers. Overall, six WSI/MPC solver combinations are compared for a heaving vertical cylinder. We also determine the pathway of energy transfer from the waves to the power take-off (PTO) system and verify the relationships using IB simulations. Additionally, three different sea states are simulated within the IB simulation to test the adaptive capability of MPC for WECs. MPC is demonstrated to adapt to changing sea conditions and find the optimal solution for each sea state.

==> Software.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\KK{Rephrase this section}
%The FD/BP algorithm and the numerical wave tank method described here is implemented within the IBAMR library~\cite{IBAMR-web-page}, which is an open-source 
%C++ simulation software focused on immersed boundary methods with adaptive mesh refinement;
%the code is publicly hosted at \url{https://github.com/IBAMR/IBAMR}.
%IBAMR relies on SAMRAI~\cite{HornungKohn02, samrai-web-page} for Cartesian grid management and the AMR framework. Linear and
%nonlinear solver support in IBAMR is provided by the PETSc library~\cite{petsc-efficient, petsc-user-ref, petsc-web-page}. All of the example cases
%in the present work made use of distributed-memory parallelism using the Message Passing Interface (MPI)
%library. 
%Simulations were carried out on both the XSEDE Comet cluster at the San Diego
%Supercomputer Center (SDSC) and the Fermi cluster at San Diego State University (SDSU).
%Comet houses 1,944 Intel Haswell standard compute nodes consisting of Intel Xeon 
%E5-2680v3 processors with a clock speed of 2.5 GHz, and 24 CPU cores per node.
%Fermi houses 45 compute nodes with different generations of Intel Xeon processors.  
%
%
%Between $64$ and $128$ cores were used for the 2D computations presented here, while $128$ cores were used for the 3D
%computations. The 2D ISWEC model using the medium grid resolution described in Sec.~\ref{subsec_grid_convergence}
%required approximately 6,129 seconds to execute 15,000 time-steps on Comet using $80$ cores. The 3D ISWEC model
%using the coarse grid resolution described in Sec.~\ref{subsec_3D_2D_models} required approximately 82,000 seconds
%to execute 10,000 time-steps on Fermi using $128$ cores of Intel Xeon E5-2697Av4 Broadwell processors with a clock speed of 2.6 GHz.
